Enumeration, structural and dimensional synthesis of robotic hands: theory and implementation

Designing robotic hands for specific tasks could help in the creation of optimized end-effectors for grasping and manipulation. However the systematic design of robotic hands for a simultaneous task of all fingertips presents many challenges. In this work the algorithms and implementation of an overall synthesis process is presented, which could be a first step towards a complete design tool for robotic end-effectors. Type synthesis for a given task and number of fingers, solvability and dimensional synthesis for arbitrary topologies are developed and implemented. The resulting solver is a powerful tool that can aid in the creation of innovative robotic hands with arbitrary number of fingers and palms. Several examples of type synthesis, solvability calculations and dimensional synthesis are presented.

==> heading.tex <==
%
\newcommand{\tin}{\mbox{\footnotesize{in}}}
\newcommand{\tout}{\mbox{\footnotesize{out}}}
\newcommand{\tA}{\mbox{\footnotesize{A}}}
\newcommand{\tB}{\mbox{\footnotesize{B}}}
\newcommand{\tC}{\mbox{\footnotesize{C}}}
\newcommand{\tO}{\mbox{\footnotesize{O}}}
\newcommand{\tft}{\mbox{\footnotesize{t}}}

\newcommand{\vectornorm}[1]{\left|\left|#1\right|\right|}

%
%unit vectors
%
\newcommand\vi{\hbox{$\vec{\imath}$}}
\newcommand\vj{\hbox{$\vec{\jmath}$}}
\newcommand\vk{\hbox{$\vec{k}$}}
\newcommand\ve{\hbox{$\vec{e}$}}
%
% bold face characters
%
\newcommand\ba{\hbox{$\bf a$}}
\newcommand\bA{\hbox{$\bf A$}}
\newcommand\bfb{\hbox{$\bf b$}}
\newcommand\bB{\hbox{$\bf B$}}
\newcommand\bc{\hbox{$\bf c$}}
\newcommand\bC{\hbox{$\bf C$}}
\newcommand\bd{\hbox{$\bf d$}}
\newcommand\bD{\hbox{$\bf D$}}
\newcommand\be{\hbox{$\bf e$}}
\newcommand\bE{\hbox{$\bf E$}}
\newcommand\ff{\hbox{$\bf f$}}
\newcommand\bF{\hbox{$\bf F$}}
\newcommand\bg{\hbox{$\bf g$}}
\newcommand\bG{\hbox{$\bf G$}}
\newcommand\bh{\hbox{$\bf h$}}
\newcommand\bH{\hbox{$\bf H$}}
\newcommand\bI{\hbox{$\bf I$}}
\newcommand\bJ{\hbox{$\bf J$}}
\newcommand\bK{\hbox{$\bf K$}}

\newcommand\bL{\hbox{$\bf L$}}
\newcommand\bbm{\hbox{$\bf m$}}
\newcommand\bM{\hbox{$\bf M$}}
\newcommand\bn{\hbox{$\bf n$}}
\newcommand\bN{\hbox{$\bf N$}}
\newcommand\bo{\hbox{$\bf o$}}
\newcommand\bO{\hbox{$\bf O$}}
\newcommand\bp{\hbox{$\bf p$}}
\newcommand\bP{\hbox{$\bf P$}}
\newcommand\bq{\hbox{$\bf q$}}
\newcommand\bQ{\hbox{$\bf Q$}}
\newcommand\br{\hbox{$\bf r$}}
\newcommand\bR{\hbox{$\bf R$}}
\newcommand\bs{\hbox{$\bf s$}}
\newcommand\bS{\hbox{$\bf S$}}
\newcommand\bt{\hbox{$\bf t$}}
\newcommand\bT{\hbox{$\bf T$}}
\newcommand\bu{\hbox{$\bf u$}}
\newcommand\bU{\hbox{$\bf U$}}
\newcommand\bv{\hbox{$\bf v$}}
\newcommand\bV{\hbox{$\bf V$}}
\newcommand\bw{\hbox{$\bf w$}}
\newcommand\bW{\hbox{$\bf W$}}
\newcommand\bx{\hbox{$\bf x$}}
\newcommand\bX{\hbox{$\bf X$}}
\newcommand\by{\hbox{$\bf y$}}
\newcommand\bY{\hbox{$\bf Y$}}
\newcommand\bz{\hbox{$\bf z$}}
\newcommand\bZ{\hbox{$\bf Z$}}
\newcommand\btheta{\mbox{\boldmath$\theta$}}
\newcommand\bomega{\mbox{\boldmath$\omega$}}
\newcommand\balpha{\mbox{\boldmath$\alpha$}}
%
% san serif characters
%
\newcommand\sA{\hbox{$\sf A$}}
\newcommand\sB{\hbox{$\sf B$}}
\newcommand\sC{\hbox{$\sf C$}}
\newcommand\sD{\hbox{$\sf D$}}
\newcommand\sE{\hbox{$\sf E$}}
\newcommand\sF{\hbox{$\sf F$}}
\newcommand\sg{\hbox{$\sf g$}}
\newcommand\sG{\hbox{$\sf G$}}
\newcommand\sH{\hbox{$\sf H$}}
\newcommand\sk{\hbox{$\sf k$}}
\newcommand\sI{\hbox{$\sf I$}}
\newcommand\sJ{\hbox{$\sf J$}}
\newcommand\sK{\hbox{$\sf K$}}
\newcommand\sL{\hbox{$\sf L$}}
\newcommand\ssl{\hbox{$\sf l$}}
\newcommand\sM{\hbox{$\sf M$}}
\newcommand\sn{\hbox{$\sf n$}}
\newcommand\sN{\hbox{$\sf N$}}
\newcommand\sO{\hbox{$\sf O$}}
%\newcommand\sp{\hbox{$\sf p$}}
\newcommand\sP{\hbox{$\sf P$}}
\newcommand\sq{\hbox{$\sf q$}}
\newcommand\sQ{\hbox{$\sf Q$}}
\newcommand\sR{\hbox{$\sf R$}}
%\newcommand\ss{\hbox{$\sf s$}}
\newcommand\sS{\hbox{$\sf S$}}
\newcommand\sT{\hbox{$\sf T$}}
\newcommand\sU{\hbox{$\sf U$}}
\newcommand\sv{\hbox{$\sf v$}}
\newcommand\sV{\hbox{$\sf V$}}
\newcommand\sw{\hbox{$\sf w$}}
\newcommand\sW{\hbox{$\sf W$}}
\newcommand\sx{\hbox{$\sf x$}}
\newcommand\sX{\hbox{$\sf X$}}
\newcommand\sy{\hbox{$\sf y$}}
\newcommand\sY{\hbox{$\sf Y$}}
\newcommand\sz{\hbox{$\sf z$}}
\newcommand\sZ{\hbox{$\sf Z$}}
%
% fractions
%
\newcommand{\divDt}{\frac{\Delta\theta}{2}}
\newcommand{\divDp}{\frac{\Delta\phi}{2}}
%
% smaller fractions
%
%\newcommand\c{\hbox{\rm c}}
\newcommand\s{\hbox{\rm s}}
\newcommand\fthetahat{\hbox{$\textstyle \frac{\hat{\theta}}{2}$}}
\newcommand\fphihat{\hbox{$\textstyle \frac{\hat{\phi}}{2}$}}
%
\newcommand\fphionehat{\hbox{$\textstyle \frac{\hat{\phi}_1}{2}$}}
\newcommand\fphitwohat{\hbox{$\textstyle \frac{\hat{\phi}_2}{2}$}}
\newcommand\fphithreehat{\hbox{$\textstyle \frac{\hat{\phi}_3}{2}$}}
%
\newcommand\fthetaone{\hbox{$\textstyle \frac {\Delta\theta_1}{2}$}}
\newcommand\fthetatwo{\hbox{$\textstyle \frac {\Delta\theta_2}{2}$}}
\newcommand\fphione{\hbox{$\textstyle \frac {\Delta\phi_1}{2}$}}
\newcommand\fphitwo{\hbox{$\textstyle \frac {\Delta\phi_2}{2}$}}
\newcommand\hatthetaone{\hbox{$\textstyle \frac {\Delta\hat{\theta}_1}{2}$}}
\newcommand\hatthetatwo{\hbox{$\textstyle \frac {\Delta\hat{\theta}_2}{2}$}}
\newcommand\hatphione{\hbox{$\textstyle \frac {\Delta\hat{\phi}_1}{2}$}}
\newcommand\hatphitwo{\hbox{$\textstyle \frac {\Delta\hat{\phi}_2}{2}$}}



\newcommand\fbeta{\hbox{$\textstyle \frac {\beta_{13}}{2}$}}
\newcommand\hatbeta{\hbox{$\textstyle \frac {\hat{\beta}_{13}}{2}$}}



